Governing Artificial Intelligence: Public Preferences and Regulatory Options

Artificial intelligence (AI) is rapidly transforming economies, societies, and polities, raising fundamental questions about how it should be regulated. Policymakers face choices over whether to prioritize innovation or safety, rely on public oversight or private self-regulation, and govern nationally or internationally. Yet little is known about how citizens evaluate these competing priorities. Here we report a conjoint survey experiment conducted in seven countries with diverse political and economic profiles. We find that citizens strongly support regulating AI and generally prioritize safety over innovation, public governance over private self-regulation, and international over national approaches. The preference for safety is strongest among those who perceive AI as risky, unpredictable, and personally consequential. These findings reveal a systematic misalignment between dominant regulatory approaches and citizen preferences.

==> tables/tab_B6_formatted.tex <==
\scriptsize
\begin{tabular}{lrrrr}
\toprule
\textbf{Country} & \textbf{Theme} & \textbf{Tasks} & \textbf{Ties} & \textbf{Tie Rate \%} \\
\midrule
Brazil & Workplace & 6198 & 0.0000 & 0.0000 \\
Brazil & Policing & 6198 & 0.0000 & 0.0000 \\
Brazil & Warfare & 6198 & 0.0000 & 0.0000 \\
China & Workplace & 6108 & 0.0000 & 0.0000 \\
China & Policing & 6108 & 0.0000 & 0.0000 \\
China & Warfare & 6108 & 0.0000 & 0.0000 \\
Germany & Workplace & 6030 & 0.0000 & 0.0000 \\
Germany & Policing & 6030 & 0.0000 & 0.0000 \\
Germany & Warfare & 6030 & 0.0000 & 0.0000 \\
India & Workplace & 6180 & 0.0000 & 0.0000 \\
India & Policing & 6180 & 0.0000 & 0.0000 \\
India & Warfare & 6180 & 0.0000 & 0.0000 \\
South Africa & Workplace & 6078 & 0.0000 & 0.0000 \\
South Africa & Policing & 6078 & 0.0000 & 0.0000 \\
South Africa & Warfare & 6078 & 0.0000 & 0.0000 \\
United Kingdom & Workplace & 6087 & 0.0000 & 0.0000 \\
United Kingdom & Policing & 6087 & 0.0000 & 0.0000 \\
United Kingdom & Warfare & 6087 & 0.0000 & 0.0000 \\
United States & Workplace & 6036 & 0.0000 & 0.0000 \\
United States & Policing & 6036 & 0.0000 & 0.0000 \\
United States & Warfare & 6036 & 0.0000 & 0.0000 \\
\bottomrule
\end{tabular}

==> tables/tab_K_ns_formatted.tex <==
\scriptsize
\begin{tabular}{lrrrr}
\toprule
\textbf{Hypothesis} & \textbf{Variable} & \textbf{N Low} & \textbf{N Neutral} & \textbf{N High} \\
\midrule
H4 & ai\_risk & 9326 & 1731 & 3182 \\
H5 & ai\_unpredictability & 4955 & 2654 & 6630 \\
H7 & internationalism & 2782 & 2351 & 9106 \\
H8 & ideology & 4431 & 1823 & 2678 \\
\bottomrule
\end{tabular}

==> tables/tab_O1_formatted.tex <==
\scriptsize
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{Term} & \textbf{Estimate} & \textbf{Std.Error} & \textbf{Statistic} & \textbf{P.Value} & \textbf{Conf.Low} & \textbf{Conf.High} & \textbf{Model} \\
\midrule
(Intercept) & 4.69 & 0.1397 & 33.56 & 0.0000 & 4.42 & 4.96 & OLS \\
country:Brazil & -0.2216 & 0.0850 & -2.61 & 0.0092 & -0.3883 & -0.0549 & OLS \\
country:China & -0.3660 & 0.0853 & -4.29 & 0.0000 & -0.5332 & -0.1988 & OLS \\
country:Germany & -0.3966 & 0.0715 & -5.54 & 0.0000 & -0.5368 & -0.2564 & OLS \\
country:India & -0.6580 & 0.1311 & -5.02 & 0.0000 & -0.9150 & -0.4011 & OLS \\
country:South Africa & -0.2901 & 0.1248 & -2.33 & 0.0201 & -0.5347 & -0.0455 & OLS \\
country:United States & -0.3354 & 0.0713 & -4.70 & 0.0000 & -0.4752 & -0.1955 & OLS \\
genderWoman & 0.0203 & 0.0531 & 0.3829 & 0.7018 & -0.0838 & 0.1244 & OLS \\
genderOther & 0.0618 & 0.1827 & 0.3380 & 0.7354 & -0.2964 & 0.4199 & OLS \\
age\_band35-49 & 0.1933 & 0.0756 & 2.56 & 0.0106 & 0.0451 & 0.3415 & OLS \\
age\_band50-64 & 0.4573 & 0.0679 & 6.73 & 0.0000 & 0.3241 & 0.5905 & OLS \\
age\_band65+ & 0.6195 & 0.0777 & 7.97 & 0.0000 & 0.4672 & 0.7718 & OLS \\
income\_3Middle & 0.3776 & 0.0561 & 6.73 & 0.0000 & 0.2675 & 0.4877 & OLS \\
income\_3High & 0.6009 & 0.0670 & 8.97 & 0.0000 & 0.4696 & 0.7323 & OLS \\
prof\_4Prof/Managers & -0.0815 & 0.0816 & -0.9986 & 0.3180 & -0.2415 & 0.0785 & OLS \\
prof\_4Skilled non-manual & -0.0067 & 0.0780 & -0.0864 & 0.9311 & -0.1596 & 0.1461 & OLS \\
prof\_4Manual & -0.0762 & 0.0844 & -0.9032 & 0.3664 & -0.2417 & 0.0892 & OLS \\
educ\_3high & 0.6551 & 0.0723 & 9.07 & 0.0000 & 0.5135 & 0.7967 & OLS \\
educ\_3middle & 0.4937 & 0.0691 & 7.14 & 0.0000 & 0.3581 & 0.6292 & OLS \\
risk\_3:Neutral & -0.0716 & 0.0693 & -1.03 & 0.3013 & -0.2075 & 0.0642 & OLS \\
risk\_3:High & 0.6129 & 0.0743 & 8.25 & 0.0000 & 0.4673 & 0.7585 & OLS \\
unpred\_3:Neutral & -0.5661 & 0.0644 & -8.79 & 0.0000 & -0.6924 & -0.4398 & OLS \\
unpred\_3:High & -0.2405 & 0.0663 & -3.63 & 0.0003 & -0.3705 & -0.1105 & OLS \\
trust\_tech\_3:Neutral & 0.0753 & 0.0686 & 1.10 & 0.2724 & -0.0591 & 0.2097 & OLS \\
trust\_tech\_3:High & 0.1062 & 0.0796 & 1.33 & 0.1825 & -0.0499 & 0.2623 & OLS \\
ai\_knowledge & 0.2408 & 0.0459 & 5.24 & 0.0000 & 0.1507 & 0.3308 & OLS \\
ideology\_3:Left & 0.0690 & 0.0575 & 1.20 & 0.2307 & -0.0438 & 0.1818 & OLS \\
ideology\_3:Right & -0.0651 & 0.0667 & -0.9767 & 0.3288 & -0.1959 & 0.0656 & OLS \\
trust\_gov\_3:Neutral & -0.0448 & 0.0680 & -0.6594 & 0.5097 & -0.1782 & 0.0885 & OLS \\
trust\_gov\_3:High & 0.1017 & 0.0796 & 1.28 & 0.2013 & -0.0543 & 0.2577 & OLS \\
\bottomrule
\end{tabular}

==> tables/tab_O2_formatted.tex <==
\scriptsize
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{Term} & \textbf{Estimate} & \textbf{Std.Error} & \textbf{Statistic} & \textbf{P.Value} & \textbf{Conf.Low} & \textbf{Conf.High} & \textbf{Model} \\
\midrule
(Intercept) & 0.6187 & 0.2357 & 2.62 & 0.0087 & 0.1567 & 1.08 & Logit \\
country:Brazil & -0.4531 & 0.1641 & -2.76 & 0.0058 & -0.7748 & -0.1314 & Logit \\
country:China & 0.1776 & 0.1771 & 1.00 & 0.3161 & -0.1696 & 0.5248 & Logit \\
country:Germany & -0.5065 & 0.1446 & -3.50 & 0.0005 & -0.7899 & -0.2231 & Logit \\
country:India & -0.8139 & 0.2093 & -3.89 & 0.0001 & -1.22 & -0.4038 & Logit \\
country:South Africa & -0.4391 & 0.2064 & -2.13 & 0.0334 & -0.8436 & -0.0346 & Logit \\
country:United States & -0.5887 & 0.1424 & -4.13 & 0.0000 & -0.8677 & -0.3096 & Logit \\
genderWoman & -0.0513 & 0.0870 & -0.5897 & 0.5554 & -0.2219 & 0.1193 & Logit \\
genderOther & 0.9130 & 0.5512 & 1.66 & 0.0976 & -0.1673 & 1.99 & Logit \\
age\_band35-49 & 0.1651 & 0.1113 & 1.48 & 0.1378 & -0.0530 & 0.3832 & Logit \\
age\_band50-64 & 0.4252 & 0.1178 & 3.61 & 0.0003 & 0.1943 & 0.6561 & Logit \\
age\_band65+ & 0.8932 & 0.1439 & 6.21 & 0.0000 & 0.6111 & 1.18 & Logit \\
income\_3Middle & 0.5119 & 0.0933 & 5.49 & 0.0000 & 0.3291 & 0.6946 & Logit \\
income\_3High & 0.9137 & 0.1132 & 8.07 & 0.0000 & 0.6918 & 1.14 & Logit \\
prof\_4Prof/Managers & -0.1714 & 0.1312 & -1.31 & 0.1915 & -0.4286 & 0.0858 & Logit \\
prof\_4Skilled non-manual & -0.0204 & 0.1219 & -0.1677 & 0.8668 & -0.2594 & 0.2185 & Logit \\
prof\_4Manual & 0.0357 & 0.1252 & 0.2854 & 0.7753 & -0.2096 & 0.2811 & Logit \\
educ\_3high & 1.01 & 0.1067 & 9.49 & 0.0000 & 0.8038 & 1.22 & Logit \\
educ\_3middle & 0.6698 & 0.0939 & 7.14 & 0.0000 & 0.4858 & 0.8537 & Logit \\
risk\_3:Neutral & -0.4619 & 0.1212 & -3.81 & 0.0001 & -0.6995 & -0.2244 & Logit \\
risk\_3:High & 0.4728 & 0.1247 & 3.79 & 0.0001 & 0.2285 & 0.7172 & Logit \\
unpred\_3:Neutral & -1.08 & 0.1174 & -9.23 & 0.0000 & -1.31 & -0.8533 & Logit \\
unpred\_3:High & -0.4548 & 0.1091 & -4.17 & 0.0000 & -0.6686 & -0.2409 & Logit \\
trust\_tech\_3:Neutral & 0.2191 & 0.1118 & 1.96 & 0.0500 & 0.0000 & 0.4381 & Logit \\
trust\_tech\_3:High & 0.2223 & 0.1179 & 1.89 & 0.0593 & -0.0087 & 0.4533 & Logit \\
ai\_knowledge & 0.4723 & 0.1130 & 4.18 & 0.0000 & 0.2508 & 0.6939 & Logit \\
ideology\_3:Left & 0.1374 & 0.0989 & 1.39 & 0.1648 & -0.0564 & 0.3312 & Logit \\
ideology\_3:Right & 0.0260 & 0.1120 & 0.2324 & 0.8162 & -0.1934 & 0.2455 & Logit \\
trust\_gov\_3:Neutral & -0.1310 & 0.1151 & -1.14 & 0.2550 & -0.3566 & 0.0946 & Logit \\
trust\_gov\_3:High & 0.0410 & 0.1208 & 0.3394 & 0.7343 & -0.1957 & 0.2777 & Logit \\
\bottomrule
\end{tabular}
